A Framework to Generate High-Quality Datapoints for Multiple Novel Intent Detection

Systems like Voice-command based conversational agents are characterized by a pre-defined set of skills or intents to perform user specified tasks. In the course of time, newer intents may emerge requiring retraining. However, the newer intents may not be explicitly announced and need to be inferred dynamically. Thus, there are two important tasks at hand (a). identifying emerging new intents, (b). annotating data of the new intents so that the underlying classifier can be retrained efficiently. The tasks become specially challenging when a large number of new intents emerge simultaneously and there is a limited budget of manual annotation. In this paper, we propose MNID (Multiple Novel Intent Detection) which is a cluster based framework to detect multiple novel intents with budgeted human annotation cost. Empirical results on various benchmark datasets (of different sizes) demonstrate that MNID, by intelligently using the budget for annotation, outperforms the baseline methods in terms of accuracy and F1-score.

==> 2Related.tex <==
\section{Related Work} 
\label{sec:related}
%\noteng{Frankly I am not seeing too much coherence, please elaborate}
In the last decade, researchers mostly focus on novel class detection in various scenarios like  out-of-domain class detection, class emergence phenomenon in streaming environment. People explore different clustering based approaches - semi-supervised or unsupervised. We review related work on the emerging new class phenomenon as well as budgeted annotation strategy to optimize human annotation effort.

%In the last decade, researchers have focused on out of domain class detection in various scenarios. People have also explored various few shot class detection approaches to get optimum accuracy with minimum labeling cost. We review related work on the novel class detection as well as few shot based strategy to optimized classification results with less human annotation effort.

%\pg{Still having a very hard time following this. Please keep this focused, connecting to your task, and mentioning limitations. You can reduce it a lot.}
%\pg{Describe the structure of this section, and then go into details. Do you need to have streaming learning as a separate subsection? Also, last subsection needs to be connected to our story, rather than generic active learning.}
%\textcolor{violet}{one option is to remove all subsection headings? or remove streaming learning heading and adding back to novel class detection}
\begin{comment}


\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|c|ccc|c|}
\hline
\multirow{2}{*}{\textbf{Dataset ($W$)}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Intent \\ Class ($|N|$)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Total \\ Data ($|W|$)\end{tabular}}} & \multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{\#Lab (|$D_{init}$|)}} & \multicolumn{3}{c|}{\textbf{\#Unlab ($|D|$ - |$D_{init}$|)}}                                                        & \multirow{2}{*}{\textbf{\#Test ($|T|$)}} \\ \cline{6-8}
                                  &                                                                                      &                                                                                 &                                &                                 & \multicolumn{1}{c|}{\textbf{\#IND}} & \multicolumn{1}{c|}{\textbf{\#OOD}} & \textbf{\#Total} &                                  \\ \hline
\multirow{3}{*}{SNIPS}            & \multirow{3}{*}{7 (5+2)}                                                             & \multirow{3}{*}{14484}                                                          & 1                              & 50                              & \multicolumn{1}{c|}{8601}           & \multicolumn{1}{c|}{3449}           & 12050            & 2384                             \\ \cline{4-9} 
                                  &                                                                                      &                                                                                 & 2                              & 50                              & \multicolumn{1}{c|}{8569}           & \multicolumn{1}{c|}{3481}           & 12050            & 2384                             \\ \cline{4-9} 
                                  &                                                                                      &                                                                                 & 3                              & 50                              & \multicolumn{1}{c|}{8629}           & \multicolumn{1}{c|}{3421}           & 12050            & 2384                             \\ \hline
\multirow{3}{*}{FB}               & \multirow{3}{*}{12 (9+3)}                                                            & 43263                                                                           & EN                             & 90                              & \multicolumn{1}{c|}{7888}           & \multicolumn{1}{c|}{26962}          & 34850            & 8323                             \\ \cline{3-9} 
                                  &                                                                                      & 8643                                                                            & ES \ddag                            & 90                              & \multicolumn{1}{c|}{1588}           & \multicolumn{1}{c|}{4321}           & 5909             & 2644                             \\ \cline{3-9} 
                                  &                                                                                      & 5083                                                                            & TH \ddag                            & 90                              & \multicolumn{1}{c|}{1113}           & \multicolumn{1}{c|}{2797}           & 3910             & 1083                             \\ \hline
ATIS                              & 17 (10+7)                                                                            & 5871                                                                            & -                              & 100                             & \multicolumn{1}{c|}{4084}           & \multicolumn{1}{c|}{686}            & 4771             & 1000                             \\ \hline
BANKING*                          & 77 (10+67)                                                                           & 13083                                                                           & -                              & 100                             & \multicolumn{1}{c|}{1026}           & \multicolumn{1}{c|}{8877}           & 9903             & 3080                             \\ \hline
CLINC*                           & 150 (10+140)                                                                         & 22500                                                                           & -                              & 100                             & \multicolumn{1}{c|}{1100}            & \multicolumn{1}{c|}{16800}           & 17900            & 4500                             \\ \hline
\end{tabular}
\caption{Dataset Statistics based on our split for various Datasets. * represents pre-defined train-test splits. (- + -) represents (known + unknown intents). {\ddag} represents Non-English datasets}
\label{tab:dataset}
\end{table*}

\end{comment}





% Please add the following required packages to your document preamble:
% \usepackage{multirow}

%\subsection{Streaming Learning}
\iffalse{}
\noindent \textbf{Out of domain Class Detection}: In dynamic and evolutionary real world applications, various flexible adaptive novel class detection models have been developed. \cite{zhou2002hybrid,kuzborskij2013n,scheirer2012toward} worked on incremental learning in dynamic environment for evolving new class. \cite{sun2016online} focused on class evolution phenomenon of emergence and disappearance of classes. %\cite{spinosa2009novelty,hayat2010dct,abdallah2016anynovel} have developed cluster based single novel class detection approaches. 
\cite{na2018dilof,ma2003time,larson2019evaluation,yan2020unknown} detect new class in the form of outlier detection. \cite{lin2019deep} built a large margin cosine loss (LMCL) based method to identify unknown intents. \cite{cavalin2020improving} use word graph embeddings to detect intents. \cite{ouyang2021energy} propose energy based score using a data manipulation framework to Generate
high-quality OOD utterances with importance
weighTs (GOT). \cite{zhan2021out} detects out of scope intents constructing a set of pseudo outliers in the training stage. FS-OOD~\cite{tan2019out} proposed a new method to tackle the OOD detection task in low-resource settings. MSP~\cite{hendrycks2018baseline}, ODIN \cite{liang2018enhancing} use softmax probability scores for out-of-domain sample detection. DeepUnk~\cite{lin2019deep} use margin loss to detect OOD.
%Protaugment~\cite{dopierre2021protaugment} is a meta-learning based intent detection algorithm to OOD detection using unsupervised diverse intent paraphrasing. 
These approaches do not distinguish among  new class labels so these are not useful for novel multi-class detection within a budgeted cost. We use FS-OOD approach in our pipeline and other methods as baseline. \noteng{Why is this paragraph important, isn't it the one already said when we are discussing the baselines}
\fi
%\subsection{Streaming Scenario}
\noindent \textbf{Streaming Scenario}
Some advanced approaches have been developed to explore novel class detection problem in data stream. ECSMiner \cite{masud2010classification} is a clustering based ensemble of classification models to resolve streaming problems. % like concept drift and concept evolution. But the time delay assumption for getting true labels and fixed size chunks are unrealistic in real world scenarios. 
SAND \cite{haque2016sand} is a semi-supervised framework to identify class boundaries by classifier confidence scores. \cite{wang2020active} used high dimensional data for streaming classification. 
Based on Frequent-Directions technique \cite{liberty2013simple}, SENC-MaS \cite{mu2017streaming} is a matrix sketch method to detect new class and update the classifier. SENCForest \cite{mu2017classification} uses random trees as a single common core to identify new classes. But both these approach rely on a large
labeled initial training set and do not use the unlabeled data. SEEN \cite{zhu2020semi} is graph-based semi-supervised classifier,
which uses both labeled and unlabeled data to
detect emerging new classes and classify known classes. \cite{spinosa2009novelty,hayat2010dct} detects novelty in  data streams. But these algorithms fail to identify multiple classes in a new stream within a particular annotation cost so these models are unable to detect multiple novel classes. %We have used SEEN, SENC-MaS and SENNE approaches as baselines.

%\subsection{Novel Class Detection}

% But these algorithms are not suitable for multiple novel-class detection and classification.%\cite{} towards classifying user queries into pre-defined intents and identifying the novel classes. 
%\subsection{Out of Domain Intent Detection}

%\cite{yan2020unknown} proposed a semantic-enhanced Gaussian Mixture Model that learns dynamic embeddings that enables downstream outlier detection. %\cite{cavalin2020improving} modeled a method based on mapping class labels to nodes in a word graph and then mapping embeddings of text to the node embeddings of classes to find the intent for that text. 
 %\cite{tan2019out} proposed a new method to tackle the OOD detection task in low-resource settings, without adversely affecting performance on the few-shot ID classification. We use this approach as baseline.


%\cite{ouyang2021energy} propose energy based score using a data manipulation framework to Generate high-quality OOD utterances with importance weighTs (GOT). Protaugment~\cite{dopierre2021protaugment} is a meta-learning based intent detection algorithm to OOD detection using unsupervised diverse intent paraphrasing. We use these two approaches as baselines. %DRM \cite{shen2021enhancing} is a novel domain regularization model to detect OOD using only in-domain data for spoken language understanding.  \cite{zhan2021out} detects out of scope intents constructing a set of pseudo outliers in the training stage. But this model requires few assumptions in data distributions and sampling which is not much practical to use.   

%\cite{hendrycks2018baseline,vyas2018out,liang2017enhancing} use softmax probability scores for out-of-domain sample detection. Though these approaches perform well but are unable to detect multiple novel classes and classify data-points as in-domain and out-of-domain. 
%\subsection{Few Shot Based Approaches}
\noindent \textbf{Clustering Based Frameworks:} Researchers work on various unsupervised and semi-supervised clustering based frameworks for new class detection. Unsupervised clustering methods K-Means~\cite{macqueen1967some}, Agglomerative clustering~\cite{gowda1978agglomerative} are explored earlier. People study different neural network based unsupervised approaches also - DCN~\cite{yang2017towards}, DEC~\cite{xie2016unsupervised}. Clustering information are also used to explore several semi-supervised models for intent detection. KCL~\cite{hsu2017learning} use domain adaptation and cross task transfer learning to conduct clustering. MCL~\cite{hsu2019multi}, CDAC+~\cite{lin2020discovering}, Deep-Aligned~\cite{zhang2021discovering} use pairwise similarity information for clustering. DTC~\cite{han2019learning} apply transfer learning on top of DEC for clustering. Our algorithm is based on K-Means clustering. We show other approaches as baselines.


\noindent \textbf{Budgeted Annotation Cost}: 
%FLEX \cite{bragg2021flex} describe Few-shot Language Evaluation across (X) many transfer types. \cite{perez2021true} propose model selection criteria (cross-validation and minimum description length) for few shot approaches. 
We explore different few shot based approaches for optimize human labeling cost. 
HAPN \cite{sun2019hierarchical} is a attention based prototypical network for few shot text classification. \cite{bao2019few} learn the model from distributional signatures, which encode pertinent word occurrence patterns. But none of these works explore novel intent class detection problem.  
IFSTC \cite{xia2021incremental} and TARS \cite{halder2020task} develop a system to classify intents with only few annotated examples per class. These approaches incrementally learn new classes. These models are working only on known classes (few examples of test classes should be present in train set for model building otherwise the system unable to identify new classes). 
%\cite{casanueva2020efficient} is a few shot based multiple intent classification framework 
But these works do not deal with the multiple unseen intent detection and classification task. %Though these approaches perform well but are unable to detect multiple novel classes. 
\pg{But why are you reviewing few-shot methods? You need to focus only on the budget constraint, and describe a few relevant approaches for your scenarios.}

==> Error.tex <==
\begin{comment}


\section{Error Analysis}



In this section, we perform an error analysis of different parts of our proposed framework to gain more insights into the difficult cases. 

%\subsection{Error Analysis}
%\noindent \textbf{Multiple Novel Intent Detection:} %We discuss some of the errors committed by our model on the various datasets. 
\noindent (i) The trained model, $\mathcal{M}$, sometimes falters when two intents are very similar. On the SNIPS dataset, the sentence "\textit{i m wondering when i can see hurry sundown}" has gold label "\textit{SearchScreeningEvent}" but the model predicts as "\textit{SearchCreativeWork}" since both are similar. %Other such example would be "give a 5 to a picture of her tombstone" should be classified as "RateBook" but the model predicts "SearchCreativeWork" because of no mention of any word related to book. 
%Also in case of facebook dataset, the sentence "remind me to set the alarm for the house tonight" is annotated as "set reminder" but the model predicts "set alarm". In case of ATIS, some of the examples such as `what is restriction ap80 ?' is annotated in the dataset as atis\_restriction which was Out-Of-Domain in our case but our OOD detection framework fails to detect this as OOD and detects it as atis\_abbreviation which is an in-domain intent for us. This as such reduces the macro-F1 for our framework.
\iffalse
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{\# MNID}} & \multirow{2}{*}{\textbf{\# ALC}} & \multirow{2}{*}{\textbf{\# Total}} & \multirow{2}{*}{\textbf{\# Unlab}} & \multirow{2}{*}{\textbf{\% annot}} \\
                                  &                                &                                   &                                  &                                    &                                    &                                    \\ \hline
\multirow{3}{*}{SNIPS}            & 1                              & 589                               & 29                               & 618                                & 9110                               & \textbf{6.78}                      \\ \cline{2-7} 
                                  & 2                              & 669                               & 43                               & 712                                & 9110                               & \textbf{7.82}                      \\ \cline{2-7} 
                                  & 3                              & 613                               & 37                               & 650                                & 9110                               & \textbf{7.14}                      \\ \hline
\multirow{3}{*}{FB}               & EN                             & 1600                              & 984                              & 2584                               & 25000                              & \textbf{10.36}                     \\ \cline{2-7} 
                                  & ES                             & 240                               & 55                               & 295                                & 4000                               & \textbf{7.38}                      \\ \cline{2-7} 
                                  & TH                             & 250                               & 54                               & 304                                & 3000                               & \textbf{10.13}                     \\ \hline
ATIS                              & -                              & 100                               & 260                              & 360                                & 3364                               & \textbf{10.70}                     \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Overall annotation requirememts \\ for MNID-ALC}
\vspace{-2mm}
\label{tab:annot_total}
\vspace{-2mm}
\end{table}
\fi


\noindent (ii) Majority Voting does not perform well in MNID because of less annotated data (novel classes) for training but it works well in ALC as training is done on more data (labelled data ($\mathcal{L}$)). 

\noindent (iii) Our OOD detection as well as clustering approaches do not perform well in case of ATIS datasets. This is due to the less amount of data and higher similarity of the known and unknown intents. For eg., detecting conjoined intents such as `atis\_ground\_service\#atis\_ground\_fare', which resemble `atis\_ground\_service' and `atis\_ground\_fare'. 

\iffalse
\noindent \textbf{Active Learning Classification: } (i) ALC is able to save significant human annotation effort but it also requires extra training cost for majority voting classifiers. 

(ii) ALC can detect known intents with better accuracy but is unable to improve accuracy of novel intent classes in that same cycle. It is likely to improve when a new set of data comes.
%\iffalse
(iii) ALC fails to maintain accuracy after 2nd cycle for ATIS Datasets because it has more number of intent classes (17). 
\fi
\end{comment}
%(iii) ALC is not an independent algorithm as it has to be used on top of a novel class detection method for out-of-domain class detection problems.

==> old-approach.tex <==
\begin{algorithm}[!thb]
\caption{OOD Detection Algorithm \\ OODD($|D_{init}|,|D|$) }
\label{algo1:mnid-alc}
\begin{algorithmic}[1]
%\State OOD Detection Algorithm \noteng{change this}
\State Train OOD-SDA on $|D_{init}|$ and predict on $(|D|-|D_{init}|)$ to get OOD samples, $\mathcal{OS}$ 
\State Return $\mathcal{OS}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!thb]
\caption{NCD($\mathcal{OS}$, $\mathcal{L}$, $N_{init}$, $N_{App}$)} 
\label{algo2:ncd}
\noteng{forget about $N_{App}$}
\begin{algorithmic}[1]
\State Start K-Means Clustering with an initial number of clusters, K== $N_{App}$.
\If{$N_{App} < 0 $}
\State K = max($N_{init}$, 1)
%\Else
%\State K = $N_{Approx}$
\EndIf
\State Cluster OS into K clusters.
\State Select x points from each cluster and annotate to find number of new classes, $N_{new}$. Add x*K point labels to $\mathcal{L}$.
\If{$N_{new}\geq K$ and $\mathcal{L}<\mathcal{B}$ and $N_{App} \leq 0$} 
    \State $K \gets 2*K$
    \State Repeat Steps 7-9
\Else
    \State $K \gets N_{new}$
    \State break
\EndIf 
\State $\mathcal{CL}$ = Store All $N_{new}$ Clusters
\State Return ($\mathcal{L}$,$N_{new}$, $\mathcal{CL}$)
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[!thb]
\caption{Cluster Quality($\mathcal{L}$,$N_{new}$, $\mathcal{CL}$)}
\label{algo3:quality_cluster}
\begin{algorithmic}[1]
\If{$\mathcal{L}<\mathcal{B}$}
\State Take p points from each of the clusters ($\mathcal{CL}$) and annotate to find Good Cluster ($G_{CL}$) and Bad Cluster($B_{CL}$). 
\State Add annotated p*$N_{new}$ point labels to $\mathcal{L}$.
\EndIf
\If{Any Bad Cluster is present and $\mathcal{L}<\mathcal{B}$} 
    \State Take q more points from Bad cluster and annotate q points. 
    \State Add q*$N_{new}$ point labels to $\mathcal{L}$.
\EndIf
\State Return($\mathcal{L}$,$N_{new}$, $G_{CL}$, $B_{CL}$)
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[!thb]
\caption{Annotation Strategy($\mathcal{L}$, $\mathcal{CL}$, $G_{CL}$, $B_{CL}$, $\mathcal{TH}1, \mathcal{TH}2  $ )}
\label{algo4:annotation}
\begin{algorithmic}[1]
\State Train Model $\mathcal{M}$ on $\mathcal{L}$ and predict on the remaining points in the clusters to get the confidence score (CS) of each data point.
    \For{Each point with CS and $\mathcal{L}<\mathcal{B}$}
    \If{$CS \geq \mathcal{TH}1 $ and point in $G_{CL}$}
    \State $L_{s} \gets$ Silver Annotation Strategy 
    \ElsIf{$CS \leq \mathcal{TH}2 $ and point in $B_{CL}$}
    \State $L_{g} \gets$ Gold Annotation Strategy
    %\Else
    %    \State Continue
    \EndIf
    \EndFor
\State $\mathcal{L} \gets$ $\mathcal{L}$ $\cup$ $L_s$ $\cup$ $L_g$
\State Return ($\mathcal{L}$)
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[!thb]
\caption{Multiple Novel Intent Detection (MNID)}
\label{algo:mnid}
\begin{algorithmic}[1]
\Input
  \Desc{$D_{init}$}{\hspace{2mm}Initial Labelled Data}
   \Desc{$N_{App}$}{\hspace{2mm}Approximate Unknown Class Count}
  \Desc{$\mathcal{TH}1$}{\hspace{2mm} Predefined Threshold}
  \Desc{$\mathcal{TH}2$}{\hspace{2mm} Predefined Threshold}
   \Desc{$\mathcal{T}$}{\hspace{2mm}Blind Test Data}
  %\Desc{$\mathcal{MV}$}{\hspace{2mm}Majority Voting Count}
  \EndInput
\Paramters
    \Desc{$|D|$}{\hspace{2mm}Total Data points}
    \Desc{$\mathcal{B}$}{\hspace{2mm}Total Budget}
    %\Desc{$\mathcal{M2}$}{Neural Model}
    %\Desc{$\mathcal{J}$}{Joint BERT Model\cite{chen2019bert}}
    \EndParameter
\Procedure{Novel Intent Detection}{}
 \State $N_{init} \gets$ Known Class Count from $|D_{init}|$
 \State $\mathcal{L} \gets |D_{init}|$
\State $\mathcal{OS} \gets$ Algo \ref{algo1:mnid-alc}
\State $\mathcal{L}$,$N_{new}$, $\mathcal{CL} \gets $ Algo \ref{algo2:ncd}
\State $\mathcal{L}$,$N_{new}$, $G_{CL}$, $B_{CL} \gets$ Algo \ref{algo3:quality_cluster}
\State $\mathcal{L} \gets$ Algo \ref{algo4:annotation}
\State Train neural model $\mathcal{M}$ on $\mathcal{L}$ and test on $\mathcal{T}$ to find out Accuracy, F1 and $N_{new}$.
\EndProcedure
\end{algorithmic}
\end{algorithm}


\iffalse{}
\begin{algorithm}[!thb]
\caption{Multiple Novel Intent Detection}
\label{algo:mnid-alc}
\begin{algorithmic}[1]
\Input
  \Desc{$\mathcal{L}$}{\hspace{2mm}Labelled Data }
  \Desc{$\mathcal{U}$}{\hspace{2mm}Unlabelled Data }
   \Desc{$\mathcal{T}$}{\hspace{2mm}Blind Test Data}
  \Desc{$\mathcal{TH}$}{\hspace{2mm}A predefined Threshold}
  %\Desc{$\mathcal{MV}$}{\hspace{2mm}Majority Voting Count}
  \EndInput
\Paramters
    \Desc{$\mathcal{M}$}{Neural Model}
    %\Desc{$\mathcal{M2}$}{Neural Model}
    %\Desc{$\mathcal{J}$}{Joint BERT Model\cite{chen2019bert}}
    \EndParameter
\Procedure{Novel Intent Detection}{}
%\For{each node $i$ \Pisymbol{psy}{206} $N$ }
%\State Train $\mathcal{M}$ on $\mathcal{L}$ and predict on $\mathrm{T}$.
\State Train OOD-SDA on $\mathcal{L}$ and predict on $\mathcal{U}$ to get OOD samples, $\mathcal{U'}$ 
\State Start K-Means Clustering with an initial number of clusters, K = max(number of known classes, 1). 
\State Cluster all the OOD data into K clusters.
\State Select x points from each cluster and annotate to find number of new classes, N. Add x point labels to $\mathcal{L}$.
\If{$N\geq K$} 
    \State $K \gets 2*K$
    \State Repeat Steps 11-14
\Else
    \State $K \gets N$
    \State break
\EndIf 
\State Take p points from each of K clusters and annotate to find Good Cluster and Bad Cluster. Add annotated p point labels to $\mathcal{L}$.
\If{Any Bad Cluster is present} 
    \State Take q more points from Bad cluster and annotate q points. Add q point labels to $\mathcal{L}$.
    \State Train Model $\mathcal{M}$ on $\mathcal{L}$ and predict on the remining points in the clusters to get the confidence score (CS) of each data point.
    \For{Each point with CS}
    \If{$CS \geq \mathcal{TH} $ and point from Good Cluster}
    \State Silver Annotation Strategy 
    \ElsIf{$CS \leq \mathcal{TH} $ and point from Bad Cluster}
    \State Gold Annotation Strategy
    %\Else
    %    \State Continue
    \EndIf
    \EndFor
\Else
    \State Do Silver Strategy for p points for each Good Cluster.
\EndIf

\EndProcedure
\end{algorithmic}
\end{algorithm}
\fi


%\vspace{-4mm}

%\section{Problem Definition}

\section{Problem Setting and Solution Overview}

{\bf Problem Setting:} Let there be a dataset, W with $N$ classes and $T$ as the test set. W - T = D is the rest of the dataset with $|D|$ datapoints. However, the value of N is not known. Out of the $|D|$ datapoints, $|D_{init}|~(<< |D|)$ labelled data of $N_{init}~( < N)$ classes are initially provided. The task is to design an algorithm to (a). detect all the remaining $N - N_{init}$ classes and (b). build  a high performing classifier considering all the detected classes. One can annotate a  limited budget ($B$ - $|D_{init}|$ ) of new datapoints to achieve the above mentioned two goals. 

\noindent{\bf Solution Overview:} 
The solution steps are as follows (a). Identify the (${\mathcal{OS}}$) datapoints which do not belong to the initial $N_{init}$ classes. (b). Use a part of the allotted budget of annotation to annotate a portion of these OOD (out of distribution) datapoints, 
the points are selected by repeatedly runnning a clustering algorithm with increasing number of clusters as input, and choosing cluster heads to identify the unknown classes. (c). Further identify the classes which are well clustered in feature space and which are not. Use another portion of the budget to increase the annotations of those not-so well formed class and then build up a classifier with all the classes. (d). Perform
a post-processing round whereby the remaining budget is spent on annotating low-confidence points and retrain the classifier. 

%First train a classifier with $|D_{init}|$ datapoints and identify the datapoints within $U' = (|D| - |D_{init}|)$ which doesn't fall into the $K_{init}$ classes.Prudent annotation of $U'$ data needs to be done to solve the above two mentioned problem.\noindent{\bf Identification of the number of New Intent.} There may or may not be a rough idea of $K$. In either cases, a simple way is to progressively cluster $U'$ with one, two, four and likewise cluster. At a round $i$, annotate $k' \times i$ datapoints and 

\iffalse{}
\textcolor{blue}{
Our aim is to detect multiple novel intents, increase the accuracy of the framework using active learning based framework with less number of annotations. \\
$M_0(L) \Rightarrow A_1$\\
$M_1(L+U`) \Rightarrow A_2$\\
$M_2$(L+U`+$U_{uncer}^{1}(U_{rem})) \Rightarrow A_3$\\
$M_(r+1)$(L+U`+ $\sum_{n=1}^{r} U_{uncer}^{n}(U_{rem})) \Rightarrow A_(r+2)$ \\
Total Annotation (TA) $\Rightarrow$ MVS + R\\
Goal: $A_1$ < $A_2$ < $A_3$ < ... < $A_{r+2}$ and
Minimize TA.
}
\fi
\section{Solution Detail}

We propose the algorithm ``MNID'' (Multiple Novel Intent Detection) which is shown in Algorithm \ref{algo:mnid}. As highlighted in overview, the algorithm consists of four sub-modules, each of them are discussed below: %In our framework, we keep adding data to the initial pool of labelled data at every step using the components discussed earlier, we call each of these model retraining steps as \textit{cycles}. 

\noindent \textbf{1. OOD Detection}: For the dataset, $D$, the module (\ref{algo1:mnid-alc}) takes as input the labelled data, $|D_{init}|$ and predicts the Out-of-Domain Samples (OOD) on the remaining data, $|D|-|D_{init}|$. We call the set of OOD samples predicted as ${\mathcal {OS}}$.

\noindent \textbf{2. Novel Class detection (NCD)}: In this sub-module (\ref{algo2:ncd}), we aim at finding all the new classes, $N_{new}. $On the OOD samples ($OS$) obtained in the previous sub-module (Algorithm \ref{algo1:mnid-alc}), we cluster all the  OOD samples using K-means. We annotate x points from each cluster to find the number of new classes, $N_{new}$. We start with K = $N_{init}$ if we donot have any approximation of the number of new classes or else K= $N_{approx}$. At every step, we double the number of clusters if $K \leq N_{new}$ and we haven't exhausted our budget, $B$. We call all the new clusters thus formed as $\mathcal{CL}$.

\noindent \textbf{3. Cluster Quality}: For all the clusters obtained in the last step, in this step (\ref{algo3:quality_cluster}) we evaluate the quality of each of these clusters. We annotate p points from each of these clusters and if all the p points belong to the same class, we term it as a good cluster or else a bad cluster. For the bad clusters, we annotate q more points. All these annotated points are then added to the labelled data, $\mathcal{L}$. All the annotations are performed within our budget, $B$. \\
\noindent \textbf{4. Annotation Strategy}: In this sub-step (\ref{algo4:annotation}), we annotate more points so as to augment data to the labelled set, $\mathcal{L}$. We devise two different strategies for annotation: (a) \textbf{Silver strategy}: In this strategy, we measure the cosine similarity of points annotated within that cluster with the various unannotated points in that cluster. If similarity of a point > predefined threshold, we label that point with its nearest similar annotated neighbour. (b) \textbf{Gold Strategy}: we select some of the points based on certain criteria and annotate those with their gold labels. For this algorithm, firstly we train a classifer with the labelled set, $\mathcal{L}$ as obtained in the last step and predict on the remaining points of the clusters to get the confidence of the datapoints. If the datapoint is from a good cluster and the confidence, CS is greater than the threshold, $\mathcal{TH}1$, we perform silver strategy and if the datapoint is  from a bad cluster and the confience, CS is less than the threshold, $\mathcal{TH}2$, we perform gold strategy. 

 %\footnote{After experiments, these values provide better outcomes.}. %(\textcolor{violet}{Have moved this part from OOD Detection since both the modules need it, is this fine?}) %\pg{But what about other languages?}\\
%\pg{First, present a top-down view. Five a diagram, and explain the pipeline. Then, you go to the individual parts.}

%\pg{Since this is already described, no need to repeat.}
%For our experiment purposes, we divide each dataset (total of train, dev and test) into 1) Labelled data for training ($\Tilde{20-25\%}$) 2) Blind Test data for evaluations only 3) rest of the dataset is used as unlabelled data.

\begin{comment}
\subsection{Novel Intent Detection} \label{sec:ood}
%With the increasing popularity of conversational systems such as Amazon's Alexa and Google's DialogueFlow, users have started relying on these systems immensely for performing various day-to-day tasks using voice interactions. Out-of-Domain intents are described as the queries that are not within the range of queries already defined for the conversational systems. Identifying Out-of-Domain (OOD) intents from a user's query as such forms a crucial part in the Natural Language Understanding Pipeline. 


%\subsection{Active Learning Based Out-Of-Domain Intent Detection Algorithm}
The architecture of above novel intent detection procedure is shown in Fig \ref{fig:al_archi_final}. The algorithm (Algo \ref{algo:mnid-alc}: steps 8-33) for our Novel Intent Detection consists of the following Steps:\\
%\begin{itemize}
    \noindent \textbf{Step 1} With the initial labelled data ($\mathcal{L}$) that consists of examples only from the set of known intents, we train a Neural Model ($\mathcal{M}$).\\% \pg{Be consistent in the usage of `validation' / `unlabeled'. Also, why do you need to predict on test set here? You don't have to bring in the test set at all in the method description, except maybe, at the end.}. 
    %We call this iteration as \textbf{Cycle 0}. In this iteration, the model is only aware of the known intents and as such labels the OOD examples incorrectly.
    %\pg{We may abstract out Cycle 0 above, and remove some part from here.}\\
    \noindent \textbf{Step 2} \textit{Out-Of-Domain Sample Detection Algorithm (OOD-SDA)}: In this step, we consider an algorithm to extract Out-Of-Domain (OOD) samples $\mathcal{U'}$ from the Unlabelled Data ($\mathcal{U}$) \\
    \noindent \textbf{Step 3} \textit{Clustering:} In this step, we perform K-means clustering on OOD samples $\mathcal{U'}$ where initial value of K = Number of known Classes. If Number of Known classes is 0 (i.e. complete unknown data) then at start, we set K = 1. We use bert-base-uncased embeddings for english datasets and bert-base-multilingual embeddings for non-english datasets\\ 
    \noindent \textbf{Step 4} \textit{Identify possible New Classes}: We select x points from each cluster and check their gold labels to find if all points are from same class or not. If the points are from different classes then we check how many new classes appear (apart from known classes). We call it as N. We add gold labels of x points to $\mathcal{L}$.
    If number of new classes (N) is more than K (cluster count) then we repeat K-means clustering approach with doubling K value ($K \gets 2*K$). We repeat step 4 until cluster count exceeds number of new class in that iteration.
    \\
    \noindent \textbf{Step 5} \textit{Good Cluster and Bad Cluster}: We select p points from each cluster and check their gold labels to decide whether they are from the same class. If all the points are from the same class, we call it a good cluster , else a bad cluster. For a bad cluster, we consider q more points. These p points from each good cluster and p+q points from each bad cluster are added to the labelled data, $\mathcal{L}$.    \\
    \noindent \textbf{Step 6} \textit{Annotation Strategies}: We use two strategies used for labelling the data: \\
    \noindent \textbf{a.} \textit{Silver Strategy}: In this strategy, we measure the cosine similarity of points annotated within that cluster with the various unannotated points in that cluster. If similarity of a point > predefined threshold, we label that point with its nearest similar annotated neighbour.\\
    \noindent \textbf{b.} \textit{Gold Strategy}: For some clusters, we may want to find gold annotation of various classes within those clusters within our Budget, $\mathcal{B}$ where $\mathcal{B}$ = T*10-(Number of training points + Number of points annotated until now in step 5) where T is the total number of classes now known.\\
    \noindent \textbf{Step 6.1}: With $\mathcal{L}$, we train classifier, $\mathcal{M}$ to find the confidence score (CS) of the classifier for each of the remaining data points within a cluster. We then set a confidence threshold, $Th$ and annotate the low confidence points within each bad cluster, $n_{low}$ within budget, $B$ and do the silver strategy as described above for the high confidence points, $n_{high}$ within each good cluster. These data $n_{low}$ and $n_{high}$ are added to the labelled set, $\mathcal{L}$  \\
    \noindent \textbf{Step 7} \textit{Model}: We re-train $\mathcal{M}$ on the modified training set ($\mathcal{L}$) and perform prediction on the Test Set. 
\end{comment}


%\end{itemize}

%\pg{Why do we call OOD-Baselines?}


\begin{comment}


\begin{figure}[!hbt]
	\centering
	\includegraphics[width=0.95\linewidth]{clustering-framework.pdf}
	%\vspace{-2mm}
	\hspace{3mm}\caption{Clustering framework for OOD intent detection}
	\label{fig:cluster-ood}
	\vspace{-2mm}
\end{figure}

\noindent The clustering based framework is shown in Fig \ref{fig:cluster-ood}.
\end{comment}



%The details of this active learning based architecture is shown in Fig \ref{fig:AL-archi}.
\begin{figure}
    \centering
    \includegraphics[width=9cm, height = 7 cm]{new_acl_fig_updated.jpg}
    %\includegraphics[width=\textwidth, height=8cm]{new_acl.jpg}
    \caption{End-to-end architecture of MNID: Multiple \\Novel Intent Detection}
    \label{fig:al_archi_final}
    \vspace{-2mm}
\end{figure}


\begin{comment}
\begin{figure}[!hbt]
	\centering
	\includegraphics[width=\linewidth]{AL-architecture.pdf}
	\vspace{-2mm}
	\caption{Active Learning based Classification Architecture}
	\label{fig:AL-archi}
	\vspace{-2mm}
\end{figure}

\end{comment}

\begin{table}[!hbt]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{DOC}}               & \multicolumn{2}{c|}{\textbf{MSP}}               & \multicolumn{2}{c|}{\textbf{LMCL}}              & \multicolumn{2}{c|}{\textbf{FS-OOD}}            \\ \cline{2-9} 
                                  & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{F1} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{F1} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{F1} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{F1} \\ \hline
SNIPS                           & \multicolumn{1}{c|}{79.33}             &       73.15      & \multicolumn{1}{c|}{78.21}             &    71.67               & \multicolumn{1}{c|}{74.67}             &     69.33     & \multicolumn{1}{c|}{75.83}         & 72.96  \\ \hline
ATIS                              & \multicolumn{1}{c|}{55.79}        & 47.22            & \multicolumn{1}{c|}{56.10}             &    44.71         & \multicolumn{1}{c|}{54.45}             &     40.61        & \multicolumn{1}{c|}{74.92}        & 68.64       \\ \hline
Fb-En                             & \multicolumn{1}{c|}{63.14}             &34.03     & \multicolumn{1}{c|}{61.97}             &    30.91 & \multicolumn{1}{c|}{56.09}             &        27.23     & \multicolumn{1}{c|}{83.20}        & 69.74       \\ \hline
Fb-Es                             & \multicolumn{1}{c|}{68.47}             &    31.68         & \multicolumn{1}{c|}{69.87}             &    30.58         & \multicolumn{1}{c|}{67.16}             &    27.26         & \multicolumn{1}{c|}{75.78}        & 65.20       \\ \hline
Fb-Th                             & \multicolumn{1}{c|}{65.06}             &35.15     & \multicolumn{1}{c|}{59.56}             &    29.85         & \multicolumn{1}{c|}{46.69}             &    20.53         & \multicolumn{1}{c|}{70.59}        & 69.35       \\ \hline
BANKING                           & \multicolumn{1}{c|}{56.27}             &    20.38         & \multicolumn{1}{c|}{52.50}             &    20.18         & \multicolumn{1}{c|}{52.87}             &    15.31         & \multicolumn{1}{c|}{73.67}        & 64.12       \\ \hline
CLINIC                            & \multicolumn{1}{c|}{54.77}             &    18.72         & \multicolumn{1}{c|}{53.36}             &      20.49       & \multicolumn{1}{c|}{54.12}             &    18.96         & \multicolumn{1}{c|}{77.66}        & 65.65       \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Results of various OOD-SDA on various datasets}
\label{tab:tab_iclr}
\end{table}

%\noindent  %is discussed below in detail:




